Erlangen Program at Large-2.5: Induced Representations and Hypercomplex Numbers

In the search for hypercomplex analytic functions on the half-plane, we review the construction of induced representations of the group G=SL(2,R). Firstly we note that G-action on the homogeneous space G/H, where H is any one-dimensional subgroup of SL(2,R), is a linear-fractional transformation on hypercomplex numbers. Thus we investigate various hypercomplex characters of subgroups H. The correspondence between the structure of the group SL(2,R) and hypercomplex numbers can be illustrated in many other situations as well. We give examples of induced representations of SL(2,R) on spaces of hypercomplex valued functions, which are unitary in some sense. Raising/lowering operators for various subgroup prompt hypercomplex coefficients as well. The paper contains both English and Russian versions. Keywords: induced representation, unitary representations, SL(2,R), semisimple Lie group, complex numbers, dual numbers, double numbers, Moebius transformations, split-complex numbers, parabolic numbers, hyperbolic numbers, raising/lowering operators, creation/annihilation operators

==> mydef.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%       $Id: mydef.tex,v 1.44 2009/12/29 11:34:38 kisilv Exp $    
%
%  File mydef.tex
%
\typeout{This is MyDef macros file}
\makeatletter
\def\ifundefined#1{\expandafter\ifx\csname#1\endcsname\relax}
\hyphenation{di-men-sio-nal}
%% Do not uncomment---does not work
%\ifundefined{tthtrue}
%  \newif\iftth
%\fi
\providecommand{\comment}[1]{}
\def\smnegskip{\mskip-0.6\thinmuskip}
\usepackage{amsfonts}
%\newlength{\curmathsize}
%
%   Objects
%
\providecommand{\algebra}[1]{\ensuremath{\mathfrak{#1}}}
\providecommand{\Heisen}[1]{{\ensuremath{\mathbb{H}^{#1}}}}
\providecommand{\hHeisen}[1]{\ensuremath{\widehat{\mathbb {H}}^{#1}}}
\providecommand{\Cliff}[2][\comment]{{\ensuremath{%
\mathcal{C}\kern-0.18em\ell(#1,#2)}}}
\providecommand{\uir}[3][0]{\ifcase #1{\rho^{#2}_{#3}}% 
\or {\breve{\rho}^{#2}_{#3}}%
\or {\tilde{\rho}^{#2}_{#3}}\fi}
%\providecommand{\Cliff}[2][\comment]{\ensuremath{\mathbf{Cl}(#1,#2)}}
\providecommand{\object}[2][\,]{\ensuremath{\mathrm{#2}#1}}
\providecommand{\Space}[3][]{\ensuremath{\mathbb{#2}^{#3}_{#1}{}}}
\providecommand{\such}{\,\mid\,}
\providecommand{\Jacobian}[1]{\ensuremath{\mathcal{J}(#1)}}
  \providecommand{\FSpace}[3][]{\ensuremath{\ifx#2l \ell_{#3}^{#1}{}\else
  #2_{#3}^{#1}{}\fi}} 
  \providecommand{\limlike}[1]{\mathop {\operator@font #1}}
  \providecommand{\loglike}[1]{\mathop {\operator@font #1}\nolimits}
\providecommand{\Quater}{\ensuremath{\mathcal{H}}}
\providecommand{\bos}{\mathcal{B}}
\ifundefined{qed}
    \DeclareMathSymbol{\qed}{0}{AMSa}{"03}
\fi
\providecommand{\SL}[1][2]{\ensuremath{\FSpace{SL}{#1}(\Space{R}{})}}
\providecommand{\SU}[1][1,1]{\ensuremath{\FSpace{SU}{}(#1)}}
%
%  Unary operations
%
\providecommand{\fourier}[1]{\ensuremath{\mathcal{F}^{#1}{}}}
\providecommand{\bra}[1]{\ensuremath{\left\langle#1\right|}}
\providecommand{\ket}[1]{\ensuremath{\left|#1\right\rangle}}
\providecommand{\Cplus}{\ensuremath{C^{+}}}
\providecommand{\Cstar}{\ensuremath{C^{*}}}
\providecommand{\onvol}{^{+}}
\providecommand{\spec}[1][]{\ensuremath{\mathbf{sp}}\,}
\providecommand{\sr}{\ensuremath{\mathbf{r}}\,}
\providecommand{\kernel}{\ensuremath{\mathbf{ker}}\,}
\providecommand{\ad}{\ensuremath{\mathbf{ad}}\,}
\providecommand{\diag}{\mathop {\operator@font diag}\nolimits}
\providecommand{\norm}[2][\relax]{\left\|#2\right\|\ifx#1\relax\else_{#1}\fi}
\providecommand{\modulus}[2][\relax]{\left| #2 \right|\ifx#1\relax\else_{#1}\fi}
\providecommand{\oper}[1]{\mathcal{#1}}
\providecommand{\rmi}{\mathrm{i}}
\providecommand{\rme}{\mathrm{e}}
\providecommand{\rmh}{\epsilon}
\providecommand{\rmp}{\varepsilon}
\providecommand{\tr}{\mathop{tr}}

%
%  Binary operations%
\providecommand{\scalar}[3][\relax]{\left\langle #2,#3 
        \right\rangle\ifx#1\relax\else_{#1}\fi}
\providecommand{\intersect}[2]{\left.#1\right|_{#2}}
\providecommand{\relstack}[2]{{\mathrel {\mathop {#1}\limits _{#2}}}}
%
%
%
\providecommand{\eqref}[1]{\textup{(\ref{#1})}}
\providecommand{\eqnright}[1]{\qquad\qquad  #1}
\providecommand{\person}[1]{\textsc{#1}}
%
%  WWW commands
%
\providecommand{\href}[2]{#2}
    %\ifundefined{MR}
        \providecommand{\MR}[1]{MR\href{http://www.ams.org/mathscinet-getitem?mr=#1}{#1}}
    %\else
    %    \renewcommand{\MR}[1]{ %\textbf{MR}~
    %\href{http://www.ams.org/mathscinet-getitem?mr=#1}{#1}}
    %\fi
  \providecommand{\Zbl}[1]{Zbl\href{http://www.emis.de:80/cgi-bin/zmen/ZMATH/en/zmathf.html?first=1&maxdocs=3&type=html&an=#1&format=complete}{#1}}

\providecommand{\myeprint}[2]{E-print: \href{#1}{\texttt{#2}}}
\providecommand{\mailto}[1]{\href{mailto:#1}{\texttt{#1}}}
\providecommand{\urltt}[1]{\href{#1}{\texttt{#1}}}
\providecommand{\wiki}[2]{\href{http://en.wikipedia.org/wiki/#1}{#2}}
\providecommand{\doi}[1]{doi: \href{http://dx.doi.org/#1}{#1}}

\newif\ifhevea
\newif\ifrawhtml
%\newenvironment{rawhtml}{\ifrawhtml}{\fi}
%
\makeatother
\endinput

